Introducing Delays in Multi-Agent Path Finding

We consider a Multi-Agent Path Finding (MAPF) setting where agents have been assigned a plan, but during its execution some agents are delayed. Instead of replanning from scratch when such a delay occurs, we propose delay introduction, whereby we delay some additional agents so that the remainder of the plan can be executed safely. We show that finding the minimum number of additional delays is APX-Hard, i.e., it is NP-Hard to find a $(1+\varepsilon)$-approximation for some $\varepsilon>0$. However, in practice we can find optimal delay-introductions using Conflict-Based Search for very large numbers of agents, and both planning time and the resulting length of the plan are comparable, and sometimes outperform the state-of-the-art heuristics for replanning.

==> sections/problem_old.tex <==

% problem formulation

\subsection{Multi Agent Path Finding (MAPF)}
Consider $n\in \bbN$ agents, acting in a directed graph $G=\tup{V, E}$ where each agent $i\in \{1,\ldots,n\}$ has a source $s_i \in V$ and a goal $g_i \in V$. 
We assume $G$ allows agents to stay in place in certain nodes (vertices), but not necessarily in all nodes (vertices).  That is because in practical applications, there are often environmental restrictions, e.g.,  not to block emergency exit doors, camera views, ``high way" intersections, etc.  Hence, $(v,v)\in E$ for all $v\in V' \subseteq V$.
A \emph{path} in $G$ is a sequence of vertices $\pi=v_1v_2\ldots v_m$  such that $(v_k, v_{k+1})\in E$ for all $1 \leq k < m$. 
% We assume that $G$ allows agents to stay in place, i.e.,  $(v,v)\in E$ for all $v\in V$.


Given paths $\pi_1=v_1v_2 \ldots v_{m}$ and $\pi_2=u_1 u_2 \ldots u_{m}$ in $G$ for some $m > 1$, we say that $\pi_1$ and $\pi_2$ are \emph{non-colliding} if the following conditions are satisfied 
for all $1\le k< m$:
\begin{enumerate} [label={(\roman*)}, leftmargin=0.5in]
    \item $v_k \neq u_k$ (i.e., no vertex collisions),
    \label{condition:collision} 
    \item $(v_k, v_{k+1}) \neq (u_{k+1}, u_k)$ (i.e., no edge collisions).
    \label{condition:edgeSwap}
\end{enumerate}
We extend the definition to paths of different lengths by truncating the longer path. Intuitively, this means that once a path ends, the respective agent ``disappears''\footnote{Changing this to have the agents remain at the target location does not impact our results in any significant way.}.



Given $n$ agents on a graph $G$ and two lists $s_1, \ldots, s_n$ 
% \ml{let's use `,' for lists, not paths}
and $g_1, \ldots, g_n$ of source and goal vertices, respectively, a \emph{plan} $P=\{\pi_1, \ldots, \pi_n\}$ is a set of 
%non-colliding 
paths such that $\pi_i$ drives agent $i$ from $s_i$ to $g_i$ for every $i\in \{1, \ldots, n\}$. A plan is called \emph{non-colliding} if $\pi_i$ and $\pi_j$ are non-colliding for all $i,j \in \{1,\ldots,n\}$ and $i \neq j$.
 The \emph{length} of the plan is the maximal length of a path in $P$.
The classical \emph{Multi-Agent Path Finding (MAPF)} problem is to find a non-colliding plan\footnote{Typically, the plan is required to be optimal with respect to some cost function, e.g., makespan or sum-of-costs.} $P$ on $G$. 

\subsection{Delays in MAPF}
Such plans are valid as long as the agents  can synchronously execute their paths, i.e., executing edges at the same time.  In reality, however, it is common that agents fall out of sync, e.g., due to delays in certain nodes or different execution times of edges in the (continuous) environment.  Such incidences may cause the plan to be no longer collision-free, in which case either a new plan needs be computed or the current plan needs to be repaired. In this work, we focus on the latter.

Consider a plan $P=\{\pi_1, \ldots, \pi_n\}$ that  contains collisions. We assume $P$ is obtained from a previously non-colliding plan $P_{old}$, and the collisions in $P$ are due to some agents experiencing delays in executing $P_{old}$.  We wish to quickly repair $P$ without increasing the total path length (sum-of-costs) by more than a given bound.  
% by maintaining topological properties of the $P$, e.g., for  the purposes of explainability.
Let $|\pi|$ denote the length of path $\pi$.  The \textit{sum-of-costs} of plan $P = \{\pi_1, \ldots, \pi_n\}$ is $\|P\| = \sum_{i=1}^n |\pi_i|$, sum of the individual path lengths in $P$. 
Given current path $P$, the sum-of-cost of the repaired path $P'$ has to be within a given bound $k \in \bbN$ of $\|P\|$, i.e., $\|P'\|-\|P\| \leq k$.  
% The problem we consider is as follows.

% \begin{problem}[Constrained Plan Repair (CPR)]
% \label{prob:cpr}
% Given directed graph $G = \tup{V,E}$, and plan $P=\{\pi_1,\ldots,\pi_n\}$ that is colliding due to delayed agents on a non-colliding plan, and a budget $k\in \bbN$, compute a plan  $P' = \{\pi'_1,\ldots,\pi'_n \}$ such that $P'$ is non-colliding and $\|P'\| - \|P\| \leq k$.
% \end{problem}


Our key idea in repairing plans is to use the topology of $P$ and resolve conflicts by allowing agents to stay in place. 
That is, we repair plan $P$ by introducing \emph{delays} - i.e., requiring some agents to remain in a certain vertex for a certain amount of time instead of advancing according to the prescribed path in $P$.
The intuition is that resources are put in generating and validating the original plan $P_{old}$.  It is hence desirable to use at least some of the properties of $P_{old}$.  By using the same paths, we gain several benefits, including inheriting the visual explainability of the original plan, i.e., the paths visually remain the same, ..., reducing computations... repeatability... ongoing MAPF... \ml{add more motivations}



% Recall that graph $G$ does not necessarily allow delay in every vertex.  In addition, a new plan cannot exceed the total path length of $P$ more than $k$.  
Furthermore, in the simplified version of the problem, delays can occur at every vertex. However, to allow for application-specific constraints, we allow the  more general setting in which delays can only occur in a subset of the vertices $V' \subset V$.  To account for that as well as the sum-of-cost constraint, we define $d$-delay paths.
Formally, given a path $\pi=v_1\ldots v_m$ and a set of \emph{delay-permitted indices} $D\subseteq \{1,\ldots, m\}$, we say that a path $\pi'$ is a \emph{$d$-delay} of $\pi$, for some $d\in \bbN$, if $\pi'=v_1v_1^{k_1}v_2v_2^{k_2}\ldots v_mv_m^{k_m}$ where $v_i^{k_i}$ means repeating $v_i$ for an additional $k_i$ times, and it holds that $\sum_{i=1}^m k_i=d$ and if $i\notin D$ then $k_i=0$. 
That is, $\pi'$ repeats some of the delay-permitted indices of $\pi$, so that the total amount of repetitions is $d$. 
% Recall that we assume the graph $G$ contains all self-loops, so $\pi'$ is a legal path. 

The formal statement of the problem is as follows.

\begin{problem}[Avoiding Collisions by Introducing Delays (\textbf{ACID})]
\label{prob:delay_introduction}
    Given a plan $P=\{\pi_1,\ldots,\pi_n\}$, sets of delay-permitted indices $D_1,\ldots,D_n$, and a budget $k\in \bbN$, decide whether there exist paths $\pi'_1,\ldots,\pi'_n$ where $\pi'_i$ is a $d_i$-delay of $\pi_i$ for each $i$, with $\sum_{i=1}^n d_i\le k$ and $P'=\{\pi'_1,\ldots, \pi'_n\}$ is non-colliding.
\end{problem}

Note that ACID is stated as a decision problem, but our ultimate goal is the planning problem, where we aim to repair plan $P$ by minimizing the total number of delays.  In what follows, we first study the computational complexity of ACID. We show that this problem is indeed hard (\NP-complete). We then proceed to show that, by using delays, we can reduce the repair problem to a small instance of MAPF, where existing algorithms can be utilized to obtain \emph{good} solutions quickly.  Further, we show that, repair-by-delay in fact reduces the problem to such a small instance of MAPF that even optimal algorithms such as (vanilla) CBS can be used to general minimum-delay plans even for very large number of agents; our experiments shows that CBS can repair a plan for 1,000 agents in seconds.




